Relation of the Relations: A New Paradigm of the Relation Extraction Problem

In natural language, often multiple entities appear in the same text. However, most previous works in Relation Extraction (RE) limit the scope to identifying the relation between two entities at a time. Such an approach induces a quadratic computation time, and also overlooks the interdependency between multiple relations, namely the relation of relations (RoR). Due to the significance of RoR in existing datasets, we propose a new paradigm of RE that considers as a whole the predictions of all relations in the same context. Accordingly, we develop a data-driven approach that does not require hand-crafted rules but learns by itself the RoR, using Graph Neural Networks and a relation matrix transformer. Experiments show that our model outperforms the state-of-the-art approaches by +1.12\% on the ACE05 dataset and +2.55\% on SemEval 2018 Task 7.2, which is a substantial improvement on the two competitive benchmarks.

==> sec/additional_secs.tex <==
\subsection{The Tradeoff between precision and recall}
\begin{table*}[!ht]
  
  \centering
  \resizebox{\textwidth}{!}{
    \begin{tabular}{l|ccc|ccc|ccc|ccc|ccc}
    \toprule
     & \multicolumn{3}{c|}{\textbf{BC\_dev}} & \multicolumn{3}{c|}{\textbf{BC\_test}} & \multicolumn{3}{c|}{\textbf{CTS}} & \multicolumn{3}{c|}{\textbf{WL}} & \multicolumn{3}{c}{\textbf{Overall}} \\
     & \textbf{P} & \textbf{R} & \textbf{Micro} & \textbf{P} & \textbf{R} & \textbf{Micro} & \textbf{P} & \textbf{R} & \textbf{Micro} & \textbf{P} & \textbf{R} & \textbf{Micro} & \textbf{P} & \textbf{R} & \textbf{Micro} \\
     \hline
     
    \textbf{$\text{\modelname{}}$}  & 76.76 & 64.25 & 69.8& 71.64 & \textbf{62.08} & 67.17& 63.52 & \textbf{60.25} & 59.5& 60.89 & \textbf{54.77} & 58.4 & 65.35
& \textbf{59.03}
& 61.69\\
    \textbf{$\text{\modelname{}}_\text{local}$}   & 77.01 & 61.69 & 68.44& \textbf{77.52} & 61.94 & 68.89& \textbf{71.95} &  57.93 & 59.87& 65.51 & 54.61 & 60.6 & \textbf{71.66}
& 58.16
& 63.12\\
    \textbf{$\text{\modelname{}}_\text{non-local}$} & 79.57 & \textbf{65.15} & \textbf{70.97}& 72.64 & 61.78 & 67.88& 69.14 & 52.84 & 58.55& 63.17 & 52.96 & 58.52 & 68.32
& 55.86
& 61.65\\
    \textbf{$\text{\modelname{}}_\text{glocal}$} & \textbf{80.30} & 62.98 & 70.36& 77.03 & 61.88 & \textbf{69.82}& 70.20 & 59.64 & \textbf{61.17}& \textbf{65.94} & 54.48 & \textbf{61.7} & 71.06

&58.67& \textbf{64.23}\\
    \bottomrule
    \end{tabular}
  }
  \caption{Precision and Recall on ACE05} \label{tab:addlabel}
\end{table*}



\begin{table}[htbp]
  \centering
    \begin{tabular}{lccc}
    \toprule
    \textbf{Model}    & \textbf{P} & \textbf{R} & \textbf{Micro} \\
    \midrule
    \multicolumn{4}{c}{\textbf{\emph{Non-ensemble models}}} \\
           \textbf{$\text{\modelname{}}$}  & 32.05 & \textbf{49.37} & 37.9 \\
           \textbf{$\text{\modelname{}}_\text{local}$}   & 39.31 & 45.3  & 39.24 \\
           \textbf{$\text{\modelname{}}_\text{non-local}$}  & 39.08 & 47.68 & 39.63 \\
           \textbf{$\text{\modelname{}}_\text{glocal}$}  & \textbf{44.24} & 46.86 & \textbf{39.74} \\
    \midrule
    \multicolumn{4}{c}{\textbf{\emph{Ensemble models}}} \\
           \textbf{E-$\text{\modelname{}}$}  & 40.77 & \textbf{54.03} & 42.39 \\
           \textbf{E-$\text{\modelname{}}_\text{local}$}    & 51.03 & 51.98 & 43.12 \\
           \textbf{E-$\text{\modelname{}}_\text{non-local}$}  & 52.31 & 51.39 & \textbf{43.98} \\
           \textbf{E-$\text{\modelname{}}_\text{glocal}$}  & \textbf{56.48} & 47.44 & 43.35 \\
    \bottomrule
    \end{tabular}%  
    \caption{Results on SemEval 2018 Task 7.2}

  \label{tab:res_semeval}%
\end{table}%

\subsection{Which model captures which feature well?}

2. example
\subsection{Ablation Study on ACE05}


\subsection{Two-Stage Training}
We study the performance of each stage in the two-stage learning on ACE05 validation set in Table~\ref{tab:ablation}. The first stage is binary classification to distinguish whether two entities have ``no-relation'' or a valid relation. In this stage, the glocal model which combines both the local learner and non-local supervisor performs the best, scoring +2.55 F1 scores higher than the base model.

We observe that in both datasets, there are a dominant number of negative labels. The experiments show that the difficulty is more in identifying whether there exists a relation, than in classifying the specific relation. So it is also worth exploring a two-stage learning strategy for local and non-local correlations. Following \cite{DBLP:journals/corr/abs-1909-11898}, in the first stage, we train an extraction model on identifying binary relations (where the ``no-relation'' label is treated as negative, and all other relations are positive). In the second stage, a classification model, which is trained to classify the different positive relations, will be applied on the samples which the extraction model in Stage 1 labels as positive. We denote the combination of a local extracting model and local classification model as \textbf{$\text{\modelname{}}_{\text{ex:local},  \text{cl:local}}$}, and the combination of a glocal extracting model and local classification model as \textbf{$\text{\modelname{}}_{\text{ex:glocal}, \text{cl:local}}$}.


% \begin{table}[!h]
%   \centering
%     \begin{tabular}{p{11.39em}p{3.0em}p{3.0em}}
%     \toprule
%      &       Macro & \multicolumn{1}{l}{Micro} \\
%     \midrule
%     \multicolumn{3}{c}{\textbf{\emph{Non-ensemble models}}}
%     \\
%      \cite{DBLP:conf/semeval/LuanOH18} & 39.1  &  \\
%           \cite{DBLP:conf/semeval/NooralahzadehOL18} & 33.6  &  \\
%           \modelname{} & 42.01 & 39.83 \\
%           {$\text{\modelname{}}_\text{local}$} & \textbf{44.04} & \textbf{40.22} \\
%           {
% $\text{\modelname{}}_\text{non-local}$} & 39.34 & 39.56 \\
%           {
% $\text{\modelname{}}_\text{glocal}$} & 41.93 & 39.48 \\
%           \midrule
%     \multicolumn{3}{c}{\textbf{\emph{Ensemble models}}}
%     \\
%     \cite{DBLP:conf/semeval/RotsztejnHZ18} & 49.3  &  \\
%     E-\modelname{} & 45.27 & 42.77 \\
%     E-$\text{\modelname{}}_\text{local}$ & \textbf{50.44} & \textbf{45.02} \\
%     E-$\text{\modelname{}}_\text{non-local}$ & 48.78 & 43.56 \\
%     E-$\text{\modelname{}}_\text{glocal}$ & 47.45 & 43.56 \\
%     E-$\text{\modelname{}}_{\text{ex:base},  \text{cl:local}}$ & 39.87  & 37.34 \\
%     E-$\text{\modelname{}}_{\text{ex:local},  \text{cl:local}}$ & 44.4  & 39.49 \\
%     E-$\text{\modelname{}}_{\text{ex:glocal},  \text{cl:local}}$ & 46.57 & 42.8 \\
     
%     \bottomrule
%     \end{tabular}
%     \caption{Results on Semeval 2018 Task 7 Subtask 2.}

%   \label{tab:semeval}
% \end{table}

% \begin{table}[!h]    

%   \centering
%     \begin{tabular}{ccc}
%     \toprule
%       & Macro F1 \\
%       \midrule
%           E-$\text{\modelname{}}_{\text{ex:local}}$   & 46.33 \\
%           E-$\text{\modelname{}}_{\text{ex:glocal}}$ & \textbf{46.87} \\
%           E-$\text{\modelname{}}_{\text{ex:base}}$ & 43.11 \\
%     \bottomrule
%     \end{tabular}%
%   \caption{Binary Result of Semeval 2018 task 7}
%   \label{tab:semeval_binary}%
% \end{table}%



==> sec/amazon_review.tex <==
In this paper, the authors propose a new formulation of Relation Extraction (RE). Typically, most previous methods treat it as independent classification tasks for each relation even when there exist many entities and multiple relations in the same text. The authors propose a novel perspective to RE, relation of the relations (RoR). They prove that the RoR phenomenon widely exists in RE data, and then propose this new formulation to treat all relation classifications in the same text as one holistic task. The authors develop a data-driven approach that does not require any hand-crafted rules but learns by itself the RoR, using Graph Neural Networks, and a matrix converter. They validated that their model can have substantial improvement on two benchmark datasets.
